Regime Transition in the Energy Cascade of Rotating Turbulence

Transition from a split to a forward kinetic energy cascade system is explored in the context of rotating turbulence using direct numerical simulations with a three-dimensional isotropic random force uncorrelated with the velocity field. Our parametric study covers confinement effects in large aspect ratio domains and a broad range of rotation rates. Results indicate that for fixed geometrical dimensions the Rossby number acts as a control parameter, whereas for a fixed Rossby number the product of the domain size along the rotation axis and forcing wavenumber governs the amount of energy that cascades inversely. The regime transition criterion hence depends on both control parameters.

==> mytexcommands.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% mytexcommands.tex :: these are shortcurts/definitions to ease the typeset of
%                      LaTeX documents
% tp/stockholm_2019
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% color definitions to match MATLAB
\definecolor{myorange}{rgb}{0.93, 0.69, 0.13}
\definecolor{mygrey}{rgb}{0.5, 0.5, 0.5}


% notes in red
\newcommand{\mynote}[1]{{\color{red}#1}}


% scalars
\newcommand{\abs}[1]{\left| #1 \right|}


% vectors
\let\vaccent=\v % rename builtin command \v{} to \vaccent{}
\renewcommand{\v}[1]{\ensuremath{\mathbf{#1}}} % for vectors
\newcommand{\gv}[1]{\ensuremath{\boldsymbol{#1}}} % for vectors
% .. norm of vector
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
% .. for vectors of Greek letters
\newcommand{\uv}[1]{\ensuremath{\mathbf{\hat{#1}}}} % for unit vector


% tensors
\newcommand{\ttensor}[1]{\mathcal{#1}}
\newcommand{\ttensors}{\textsuperscript}


% Fourier related
\newcommand{\fcoef}[2]{\hat{#1}_{#2}}
% nice F for Fourier transform
\newcommand{\Ftrans}[1]{\mathcal{F}\left\{#1\right\}}


% inline fractions
\newcommand{\fracinline}[2]{{{#1}}\scalebox{1.25}{/}{{#2}}}
% .. to be used in figure caption's
\newcommand{\fracinlinecap}[2]{{{#1}}\scalebox{1}{/}{{#2}}}


% mean operators
\newcommand{\mean}[1]{\langle #1 \rangle}
\newcommand{\boxmean}[1]{\left\langle #1 \right\rangle_\mathcal{L}}
\newcommand{\meanBig}[1]{\left< #1 \right>}


% derivatives
\let\underdot=\d % rename builtin command \d{} to \underdot{}
\renewcommand{\d}[2]{\dfrac{\mbox{d}{#1}}{\mbox{d}{#2}}}
\newcommand{\dd}[2]{\frac{d^2 #1}{d #2^2}} % for double derivatives
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\pdd}[2]{\frac{\partial^2 #1}{\partial #2^2}}
% .. material derivative
\newcommand{\D}[2]{\dfrac{\mbox{D}{#1}}{\mbox{D}{#2}}}
% .. inline operators
\newcommand{\pdinline}[2]{{\partial{#1}}/{\partial{#2}}}
\newcommand{\dinline}[2]{{\mbox{d}{#1}}/{\mbox{d}{#2}}}
% .. thermodynamic partial derivatives
\newcommand{\pdc}[3]{\left( \frac{\partial #1}{\partial #2}\right)_{#3}}


% integrals
\newcommand{\diff}{\mathop{}\!\mathrm{d}}
\newcommand{\Diff}[1]{\mathop{}\!\mathrm{d^#1}}
\newcommand{\ddfrac}[2]{\frac{\displaystyle #1}{\displaystyle #2}}


% gradient, divergence and curl
\newcommand{\grad}[1]{\gv{\nabla} #1}
\let\divsymb=\div % rename builtin command \div to \divsymb
\renewcommand{\div}[1]{\gv{\nabla} \cdot \v{#1}} % for divergence
\newcommand{\curl}[1]{\gv{\nabla} \times \v{#1}} % for curl


% line types
% .. solid lines
\newcommand\solidrule[1][0.3cm]{\rule[0.5ex]{#1}{.8pt}}
\newcommand{\blackline} {{\color{black}\solidrule}}
\newcommand{\redline} {{\color{red}\solidrule}}
\newcommand{\greenline} {{\color{green}\solidrule}}
\newcommand{\blueline} {{\color{blue}\solidrule}}
\newcommand{\orangeline} {{\color{myorange}\solidrule}}
\newcommand{\greyline} {{\color{mygrey}\solidrule}}
% .. dashed lines (simple)
\newcommand\dashedrule{\mbox{%
\solidrule[1mm]\hspace{.5mm}\solidrule[1mm]\hspace{.5mm}\solidrule[1mm]}}
\newcommand{\reddashedline} {{\color{red}\dashedrule}}
\newcommand{\blackdashedline} {{\color{black}\dashedrule}}
\newcommand{\greendashedline} {{\color{green}\dashedrule}}
\newcommand{\bluedashedline} {{\color{blue}\dashedrule}}
\newcommand{\orangedashedline} {{\color{myorange}\dashedrule}}
\newcommand{\greydashedline} {{\color{mygrey}\dashedrule}}
% .. dashed lines (dash,short,dash)
\newcommand\dashedtworule{\mbox{%
\solidrule[2mm]\hspace{.5mm}\solidrule[1mm]\hspace{.5mm}\solidrule[2mm]}}
\newcommand{\reddashedtwoline} {{\color{red}\dashedtworule}}
\newcommand{\blackdashedtwoline} {{\color{black}\dashedtworule}}
\newcommand{\greydashedtwoline} {{\color{mygrey}\dashedtworule}}
% .. dashed lines (dash,dash,dash)
\newcommand\dashedthreerule{\mbox{%
\solidrule[.3mm]\hspace{.25mm}\solidrule[.3mm]\hspace{.25mm}%
\solidrule[.3mm]\hspace{.25mm}\solidrule[.3mm]\hspace{.25mm}%
\solidrule[.3mm]\hspace{.25mm}\solidrule[.3mm]}}
\newcommand{\blackdashedthreeline} {{\color{black}\dashedthreerule}}

% markers
% .. filled circle
\newcommand{\blackcircle} {{\color{black}\textbullet}}
\newcommand{\bluecircle} {{\color{blue}$\bullet$}}
% .. open circle
\newcommand{\opencircle} {{\color{black}$\boldsymbol\circ$}}
\newcommand{\opencircleblue} {{\color{blue}$\boldsymbol\circ$}}
\newcommand{\opencirclered} {{\color{red}$\boldsymbol{\circ}$}}
\newcommand{\opencircleorange} {{\color{myorange}$\boldsymbol{\circ}$}}
% .. filled square
\newcommand{\filledbluesquare} {{\color{blue}$\blacksquare$}}
\newcommand{\filledblacksquare} {$\blacksquare$}
\newcommand{\filledredsquare} {{\color{red}$\blacksquare$}}
\newcommand{\filledorangesquare} {{\color{myorange}$\blacksquare$}}
\newcommand{\filledgreysquare} {{\color{mygrey}$\blacksquare$}}
% .. open square
\newcommand{\opensquare} {{\color{black}$\square$}}
\newcommand{\openredsquare} {{\color{red}$\square$}}
% .. filled triangle
\newcommand{\triangr} {{\color{black}$\blacktriangleright$}}
\newcommand{\greytriangr} {{\color{mygrey}$\triangleright$}}
% .. open triangule up
\newcommand{\opentriangleup} {{\color{black}$\triangle$}}
\newcommand{\openbluetriangleup} {{\color{blue}$\triangle$}}
\newcommand{\opengreytriangleup} {{\color{mygrey}$\triangle$}}
% .. crosses
\newcommand{\blackcross} {{\color{black}\textbf{+}}}
\newcommand{\greycross} {{\color{mygrey}\textbf{+}}}
% .. osango
\newcommand{\losango} {{\color{black}$\diamond$}}
% .. star
\newcommand{\bluestar} {{\color{blue}$*$}}


% shortcuts
% .. vertical parallel lines same size as \perp
\newcommand{\mypara}{{\mkern3mu\protect\vphantom
                     {\perp}\vrule depth 0pt\mkern2mu\vrule depth 0pt\mkern3mu}}

% .. physical quantities
% .... velocity
\newcommand{\umean}[1]{\mean{u_#1}}
\newcommand{\ufluc}[1]{u_#1'}
\newcommand{\urms}{u'}
\newcommand{\ui}{u_i}
\newcommand{\uj}{u_j}
% .... vorticity
\newcommand{\vort}{\gv{\omega}}
% .... dissipation
\newcommand{\dissip}{\varepsilon}
\newcommand{\dissipinv}{\dissip_{inv}}
\newcommand{\dissipnu}{\dissip_{\nu}}
\newcommand{\dissipI}{\dissip_{I}}
% .... energy
\newcommand{\ken}{k}
\newcommand{\kenfrisch}{K}
% .... enstrophy
\newcommand{\enstrophy}{\mathcal{E}}
% .... reynolds stresses
\newcommand{\rst}[2]{\mean{u_#1' u_#2'}}
% .... two-point correlation
\newcommand{\rpp}{r_\perp}
\newcommand{\rpar}{r_\mypara}
\newcommand{\rcyl}{\rpp,\rpar}

% .. mathematical quantities
% ... geometry
\newcommand{\dpp}{\mathcal{L}_\perp}
\newcommand{\dpar}{\mathcal{L}_\mypara}
% ...  wavenumbers of all kinds
\newcommand{\wn}{\kappa}
\newcommand{\wnv}{\gv{\kappa}}
\newcommand{\wnnorm}{\norm{\wnv}}
\newcommand{\wnnormsimp}{\wn}
\newcommand{\wnpp}{\wn_\perp}
\newcommand{\wnpar}{\wn_\mypara}
\newcommand{\wncyl}{\wnpp,\wnpar}
\newcommand{\wndpp}{\wn_f \mathcal{L}_\perp}
\newcommand{\wndpar}{\wn_f \mathcal{L}_\mypara}
\newcommand{\wnlpp}{\wn_f \ell_\perp}
\newcommand{\wnlpar}{\wn_f \ell_\mypara}
\newcommand{\kkolmo}{\wn_{\eta}}
\newcommand{\kzeman}{\wn_{\Omega}}
\newcommand{\wnf}{\wn_f}
% ... scales (velocity,length...)
\newcommand{\lscale}{l_0}
\newcommand{\lf}{\ell_f}
\newcommand{\tf}{\tau_f}
\newcommand{\ts}{\tau_s}
\newcommand{\trelax}{\tau_3}
\newcommand{\tnl}{\tau_{nl}}
\newcommand{\tnliso}{\tnl^{\,\text{iso}}}
\newcommand{\lkolmo}{\eta}
\newcommand{\tomg}{\tau_\Omega}
\newcommand{\twave}{\tau_w}
\newcommand{\uf}{u_f}
\newcommand{\uscale}{u_0}
\newcommand{\uell}{u_\ell}
\newcommand{\lpp}{\ell_\perp}
\newcommand{\lpar}{\ell_\mypara}
\newcommand{\intlscale}[2]{L^{#1}(#2)}
\newcommand{\intlscalevel}[2]{L^{#1}_{#2}}
% .... auxiliary wavenumbers
\newcommand{\wntwo}{\wn'}
\newcommand{\wntwov}{\gv{\wntwo}}
\newcommand{\wnthree}{\wn''}
\newcommand{\wnthreev}{\gv{\wnthree}}
% .... constants
\newcommand{\ceps}{C_\varepsilon}
\newcommand{\cepsiso}{\ceps^{\,\text{iso}}}
% .. acronyms
\newcommand{\turbo}{\texttt{TurBo} }
\newcommand{\inca}{\texttt{INCA}}
% .. non-dimensional numbers
% \newcommand{\reynolds}{Re}
% \newcommand{\rossby}{Ro}
% \newcommand{\reynoldslmbda}{Re_{\lambda}}
% \newcommand{\reynoldseps}{Re_{\varepsilon}}
% \newcommand{\rossbyL}{Ro^L}
% \newcommand{\rossbyw}{Ro^{\omega}}
% \newcommand{\rossbyeps}{Ro_{\varepsilon}}
% \newcommand{\rossbylmbda}{Ro_{\lambda}}
% .. non-dimensional numbers (roman)
\newcommand{\romanreynoldseps}{\mathrm{Re_{\varepsilon}}}
\newcommand{\romanreynoldslmbda}{\mathrm{Re_{\lambda}}}
\newcommand{\romanrossbyeps}{\mathrm{Ro_{\varepsilon}}}
\newcommand{\romanrossbylmbda}{\mathrm{Ro_{\lambda}}}
% .. les modelling
% .... filter
\newcommand{\filter}[1]{\widetilde{#1}}
% .... german filter operator
\newcommand{\gcm}{\mathcal{G}}
% .... sgs quantities
\newcommand{\sgstress}{\tau}
\newcommand{\sgvec}{h}
% .... strain rate /rotation tensor
\newcommand{\fs}[1]{\filter{S}_{#1}}
\newcommand{\fo}[1]{\filter{\Omega}_{#1}}


% legacy (probably from MU)
% \newcommand{\ket}[1]{\left| #1 \right>} % for Dirac bras
% \newcommand{\bra}[1]{\left< #1 \right|} % for Dirac kets
% \newcommand{\braket}[2]{\left< #1 \vphantom{#2} \right|
%  \left. #2 \vphantom{#1} \right>} % for Dirac brackets
% \newcommand{\matrixel}[3]{\left< #1 \vphantom{#2#3} \right|
%  #2 \left| #3 \vphantom{#1#2} \right>} % for Dirac matrix elements
% \let\baraccent=\= % rename builtin command \= to \baraccent
% \renewcommand{\=}[1]{\stackrel{#1}{=}} % for putting numbers above =
% \providecommand{\wave}[1]{\v{\tilde{#1}}}
% \providecommand{\fr}{\frac}
% \providecommand{\RR}{\mathbb{R}}
% \providecommand{\NN}{\mathbb{N}}
% \providecommand{\seq}{\subseteq}
% \providecommand{\e}{\epsilon}
% %
% \newtheorem{prop}{Proposition}
% \newtheorem{thm}{Theorem}[section]
% \newtheorem{axiom}{Axiom}[section]
% \newtheorem{problem}{Problem}[section]
% \usepackage{cancel}


==> tmp/_2019_04_02/mytexcommands.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% mytexcommands.tex :: these are shortcurts/definitions to ease the typeset of
%                      LaTeX documents
% tp/stockholm_2019
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% color definitions to match MATLAB
\definecolor{myorange}{rgb}{0.93, 0.69, 0.13}
\definecolor{mygrey}{rgb}{0.5, 0.5, 0.5}


% notes in red
\newcommand{\mynote}[1]{{\color{red}#1}}


% scalars
\newcommand{\abs}[1]{\left| #1 \right|}


% vectors
\let\vaccent=\v % rename builtin command \v{} to \vaccent{}
\renewcommand{\v}[1]{\ensuremath{\mathbf{#1}}} % for vectors
\newcommand{\gv}[1]{\ensuremath{\boldsymbol{#1}}} % for vectors
% .. norm of vector
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
% .. for vectors of Greek letters
\newcommand{\uv}[1]{\ensuremath{\mathbf{\hat{#1}}}} % for unit vector


% tensors
\newcommand{\ttensor}[1]{\mathcal{#1}}
\newcommand{\ttensors}{\textsuperscript}


% Fourier related
\newcommand{\fcoef}[2]{\hat{#1}_{#2}}
% nice F for Fourier transform
\newcommand{\Ftrans}[1]{\mathcal{F}\left\{#1\right\}}


% inline fractions
\newcommand{\fracinline}[2]{{{#1}}\scalebox{1.25}{/}{{#2}}}
% .. to be used in figure caption's
\newcommand{\fracinlinecap}[2]{{{#1}}\scalebox{1}{/}{{#2}}}


% mean operators
\newcommand{\mean}[1]{\langle #1 \rangle}
\newcommand{\boxmean}[1]{\left\langle #1 \right\rangle_\mathcal{L}}
\newcommand{\meanBig}[1]{\left< #1 \right>}


% derivatives
\let\underdot=\d % rename builtin command \d{} to \underdot{}
\renewcommand{\d}[2]{\dfrac{\mbox{d}{#1}}{\mbox{d}{#2}}}
\newcommand{\dd}[2]{\frac{d^2 #1}{d #2^2}} % for double derivatives
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\pdd}[2]{\frac{\partial^2 #1}{\partial #2^2}}
% .. material derivative
\newcommand{\D}[2]{\dfrac{\mbox{D}{#1}}{\mbox{D}{#2}}}
% .. inline operators
\newcommand{\pdinline}[2]{{\partial{#1}}/{\partial{#2}}}
\newcommand{\dinline}[2]{{\mbox{d}{#1}}/{\mbox{d}{#2}}}
% .. thermodynamic partial derivatives
\newcommand{\pdc}[3]{\left( \frac{\partial #1}{\partial #2}\right)_{#3}}


% integrals
\newcommand{\diff}{\mathop{}\!\mathrm{d}}
\newcommand{\Diff}[1]{\mathop{}\!\mathrm{d^#1}}
\newcommand{\ddfrac}[2]{\frac{\displaystyle #1}{\displaystyle #2}}


% gradient, divergence and curl
\newcommand{\grad}[1]{\gv{\nabla} #1}
\let\divsymb=\div % rename builtin command \div to \divsymb
\renewcommand{\div}[1]{\gv{\nabla} \cdot \v{#1}} % for divergence
\newcommand{\curl}[1]{\gv{\nabla} \times \v{#1}} % for curl


% line types
% .. solid lines
\newcommand\solidrule[1][0.3cm]{\rule[0.5ex]{#1}{.8pt}}
\newcommand{\blackline} {{\color{black}\solidrule}}
\newcommand{\redline} {{\color{red}\solidrule}}
\newcommand{\greenline} {{\color{green}\solidrule}}
\newcommand{\blueline} {{\color{blue}\solidrule}}
\newcommand{\orangeline} {{\color{myorange}\solidrule}}
\newcommand{\greyline} {{\color{mygrey}\solidrule}}
% .. dashed lines (simple)
\newcommand\dashedrule{\mbox{%
\solidrule[1mm]\hspace{.5mm}\solidrule[1mm]\hspace{.5mm}\solidrule[1mm]}}
\newcommand{\reddashedline} {{\color{red}\dashedrule}}
\newcommand{\blackdashedline} {{\color{black}\dashedrule}}
\newcommand{\greendashedline} {{\color{green}\dashedrule}}
\newcommand{\bluedashedline} {{\color{blue}\dashedrule}}
\newcommand{\orangedashedline} {{\color{myorange}\dashedrule}}
\newcommand{\greydashedline} {{\color{mygrey}\dashedrule}}
% .. dashed lines (dash,short,dash)
\newcommand\dashedtworule{\mbox{%
\solidrule[2mm]\hspace{.5mm}\solidrule[1mm]\hspace{.5mm}\solidrule[2mm]}}
\newcommand{\reddashedtwoline} {{\color{red}\dashedtworule}}
\newcommand{\blackdashedtwoline} {{\color{black}\dashedtworule}}
\newcommand{\greydashedtwoline} {{\color{mygrey}\dashedtworule}}
% .. dashed lines (dash,dash,dash)
\newcommand\dashedthreerule{\mbox{%
\solidrule[.3mm]\hspace{.25mm}\solidrule[.3mm]\hspace{.25mm}%
\solidrule[.3mm]\hspace{.25mm}\solidrule[.3mm]\hspace{.25mm}%
\solidrule[.3mm]\hspace{.25mm}\solidrule[.3mm]}}
\newcommand{\blackdashedthreeline} {{\color{black}\dashedthreerule}}

% markers
% .. filled circle
\newcommand{\blackcircle} {{\color{black}\textbullet}}
\newcommand{\bluecircle} {{\color{blue}$\bullet$}}
% .. open circle
\newcommand{\opencircle} {{\color{black}$\boldsymbol\circ$}}
\newcommand{\opencircleblue} {{\color{blue}$\boldsymbol\circ$}}
\newcommand{\opencirclered} {{\color{red}$\boldsymbol{\circ}$}}
\newcommand{\opencircleorange} {{\color{myorange}$\boldsymbol{\circ}$}}
% .. filled square
\newcommand{\filledbluesquare} {{\color{blue}$\blacksquare$}}
\newcommand{\filledblacksquare} {$\blacksquare$}
\newcommand{\filledredsquare} {{\color{red}$\blacksquare$}}
\newcommand{\filledorangesquare} {{\color{myorange}$\blacksquare$}}
\newcommand{\filledgreysquare} {{\color{mygrey}$\blacksquare$}}
% .. open square
\newcommand{\opensquare} {{\color{black}$\square$}}
\newcommand{\openredsquare} {{\color{red}$\square$}}
% .. filled triangle
\newcommand{\triangr} {{\color{black}$\blacktriangleright$}}
\newcommand{\greytriangr} {{\color{mygrey}$\triangleright$}}
% .. open triangule up
\newcommand{\opentriangleup} {{\color{black}$\triangle$}}
\newcommand{\openbluetriangleup} {{\color{blue}$\triangle$}}
\newcommand{\opengreytriangleup} {{\color{mygrey}$\triangle$}}
% .. crosses
\newcommand{\blackcross} {{\color{black}\textbf{+}}}
\newcommand{\greycross} {{\color{mygrey}\textbf{+}}}
% .. osango
\newcommand{\losango} {{\color{black}$\diamond$}}
% .. star
\newcommand{\bluestar} {{\color{blue}$*$}}


% shortcuts
% .. vertical parallel lines same size as \perp
\newcommand{\mypara}{{\mkern3mu\protect\vphantom
                     {\perp}\vrule depth 0pt\mkern2mu\vrule depth 0pt\mkern3mu}}

% .. physical quantities
% .... velocity
\newcommand{\umean}[1]{\mean{u_#1}}
\newcommand{\ufluc}[1]{u_#1'}
\newcommand{\urms}{u'}
\newcommand{\ui}{u_i}
\newcommand{\uj}{u_j}
% .... vorticity
\newcommand{\vort}{\gv{\omega}}
% .... dissipation
\newcommand{\dissip}{\varepsilon}
\newcommand{\dissipinv}{\dissip_{inv}}
\newcommand{\dissipnu}{\dissip_{\nu}}
\newcommand{\dissipI}{\dissip_{I}}
% .... energy
\newcommand{\ken}{k}
\newcommand{\kenfrisch}{K}
% .... enstrophy
\newcommand{\enstrophy}{\mathcal{E}}
% .... reynolds stresses
\newcommand{\rst}[2]{\mean{u_#1' u_#2'}}
% .... two-point correlation
\newcommand{\rpp}{r_\perp}
\newcommand{\rpar}{r_\mypara}
\newcommand{\rcyl}{\rpp,\rpar}

% .. mathematical quantities
% ... geometry
\newcommand{\dpp}{\mathcal{L}_\perp}
\newcommand{\dpar}{\mathcal{L}_\mypara}
% ...  wavenumbers of all kinds
\newcommand{\wn}{\kappa}
\newcommand{\wnv}{\gv{\kappa}}
\newcommand{\wnnorm}{\norm{\wnv}}
\newcommand{\wnnormsimp}{\wn}
\newcommand{\wnpp}{\wn_\perp}
\newcommand{\wnpar}{\wn_\mypara}
\newcommand{\wncyl}{\wnpp,\wnpar}
\newcommand{\wndpp}{\wn_f \mathcal{L}_\perp}
\newcommand{\wndpar}{\wn_f \mathcal{L}_\mypara}
\newcommand{\wnlpp}{\wn_f \ell_\perp}
\newcommand{\wnlpar}{\wn_f \ell_\mypara}
\newcommand{\kkolmo}{\wn_{\eta}}
\newcommand{\kzeman}{\wn_{\Omega}}
\newcommand{\wnf}{\wn_f}
% ... scales (velocity,length...)
\newcommand{\lscale}{l_0}
\newcommand{\lf}{\ell_f}
\newcommand{\tf}{\tau_f}
\newcommand{\ts}{\tau_s}
\newcommand{\trelax}{\tau_3}
\newcommand{\tnl}{\tau_{nl}}
\newcommand{\tnliso}{\tnl^{\,\text{iso}}}
\newcommand{\lkolmo}{\eta}
\newcommand{\tomg}{\tau_\Omega}
\newcommand{\twave}{\tau_w}
\newcommand{\uf}{u_f}
\newcommand{\uscale}{u_0}
\newcommand{\uell}{u_\ell}
\newcommand{\lpp}{\ell_\perp}
\newcommand{\lpar}{\ell_\mypara}
\newcommand{\intlscale}[2]{L^{#1}(#2)}
\newcommand{\intlscalevel}[2]{L^{#1}_{#2}}
% .... auxiliary wavenumbers
\newcommand{\wntwo}{\wn'}
\newcommand{\wntwov}{\gv{\wntwo}}
\newcommand{\wnthree}{\wn''}
\newcommand{\wnthreev}{\gv{\wnthree}}
% .... constants
\newcommand{\ceps}{C_\varepsilon}
\newcommand{\cepsiso}{\ceps^{\,\text{iso}}}
% .. acronyms
\newcommand{\turbo}{\texttt{TurBo} }
\newcommand{\inca}{\texttt{INCA}}
% .. non-dimensional numbers
% \newcommand{\reynolds}{Re}
% \newcommand{\rossby}{Ro}
% \newcommand{\reynoldslmbda}{Re_{\lambda}}
% \newcommand{\reynoldseps}{Re_{\varepsilon}}
% \newcommand{\rossbyL}{Ro^L}
% \newcommand{\rossbyw}{Ro^{\omega}}
% \newcommand{\rossbyeps}{Ro_{\varepsilon}}
% \newcommand{\rossbylmbda}{Ro_{\lambda}}
% .. non-dimensional numbers (roman)
\newcommand{\romanreynoldseps}{\mathrm{Re_{\varepsilon}}}
\newcommand{\romanreynoldslmbda}{\mathrm{Re_{\lambda}}}
\newcommand{\romanrossbyeps}{\mathrm{Ro_{\varepsilon}}}
\newcommand{\romanrossbylmbda}{\mathrm{Ro_{\lambda}}}
% .. les modelling
% .... filter
\newcommand{\filter}[1]{\widetilde{#1}}
% .... german filter operator
\newcommand{\gcm}{\mathcal{G}}
% .... sgs quantities
\newcommand{\sgstress}{\tau}
\newcommand{\sgvec}{h}
% .... strain rate /rotation tensor
\newcommand{\fs}[1]{\filter{S}_{#1}}
\newcommand{\fo}[1]{\filter{\Omega}_{#1}}


% legacy (probably from MU)
% \newcommand{\ket}[1]{\left| #1 \right>} % for Dirac bras
% \newcommand{\bra}[1]{\left< #1 \right|} % for Dirac kets
% \newcommand{\braket}[2]{\left< #1 \vphantom{#2} \right|
%  \left. #2 \vphantom{#1} \right>} % for Dirac brackets
% \newcommand{\matrixel}[3]{\left< #1 \vphantom{#2#3} \right|
%  #2 \left| #3 \vphantom{#1#2} \right>} % for Dirac matrix elements
% \let\baraccent=\= % rename builtin command \= to \baraccent
% \renewcommand{\=}[1]{\stackrel{#1}{=}} % for putting numbers above =
% \providecommand{\wave}[1]{\v{\tilde{#1}}}
% \providecommand{\fr}{\frac}
% \providecommand{\RR}{\mathbb{R}}
% \providecommand{\NN}{\mathbb{N}}
% \providecommand{\seq}{\subseteq}
% \providecommand{\e}{\epsilon}
% %
% \newtheorem{prop}{Proposition}
% \newtheorem{thm}{Theorem}[section]
% \newtheorem{axiom}{Axiom}[section]
% \newtheorem{problem}{Problem}[section]
% \usepackage{cancel}

